Pull-Push Method: A new approach to Edge-Isoperimetric Problems

We prove a generalization of the Ahlswede-Cai local-global principle. A new technique to handle edge-isoperimetric problems is introduced which we call the pull-push method. Our main result includes all previously published results in this area as special cases with the only exception of the edge-isoperimetric problem for grids. With this we partially answer a question of Harper on local-global principles. We also describe a strategy for further generalization of our results so that the case of grids would be covered, which would completely settle Harper's question.

==> authors.tex <==
%auto-ignore
\author[label1]{Sergei L. Bezrukov}
\ead{sbezruko@uwsuper.edu}
\affiliation[label1]{organization={Department of Math and Computer Science, University of Wisconsin - Superior},
	addressline={801 N28th Street},
	city={Superior},
	postcode={54880},
	state={WI},
	country={USA}}


\author[label2]{Nikola Kuzmanovski\corref{mycorrespondingauthor}}
\ead{nikola.kuzmanovski@huskers.unl.edu}
\cortext[mycorrespondingauthor]{Corresponding author}
\affiliation[label2]{organization={Department of Mathematics, University of Nebraska - Lincoln},
	addressline={210 Avery Hall, 1144 T St},
	city={Lincoln},
	postcode={68588},
	state={NE},
	country={USA}}


\author[label3]{Jounglag Lim}
\ead{joungll@clemson.edu}
\affiliation[label3]{organization={School of Mathematical and Statistical Sciences, Clemson University},
	addressline={O-110 Martin Hall, 220 Parkway Drive},
	city={Clemson},
	postcode={29631},
	state={SC},
	country={USA}}

